Computing Robust Forward Invariant Sets of Multidimensional Non-linear Systems via Geometric Deformation of Polytopes

This paper develops and implements an algorithm to compute sequences of polytopic Robust Forward Invariant Sets (RFIS) that can parametrically vary in size between the maximal and minimal RFIS of a nonlinear dynamical system. This is done through a novel computational approach that geometrically deforms a polytope into an invariant set using a sequence of homeomorphishms, based on an invariance condition that only needs to be satisfied at a finite set of test points. For achieving this, a fast computational test is developed to establish if a given polytopic set is an RFIS. The geometric nature of the proposed approach makes it applicable for arbitrary Lipschitz continuous nonlinear systems in the presence of bounded additive disturbances. The versatility of the proposed approach is presented through simulation results on a variety of nonlinear dynamical systems in two and three dimensions, for which, sequences of invariant sets are computed.

==> bio-Taha_Ameen.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%------------------------- Taha Ameen ------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Author_Biographies/Taha_Picture.jpg}}]{Taha Ameen}  

\end{IEEEbiography}
%%\vspace{-5 mm}
%%%======================================
